JWST reveals a possible $z \sim 11$ galaxy merger in triply-lensed MACS0647$-$JD

MACS0647$-$JD is a triply-lensed $z\sim11$ galaxy originally discovered with the Hubble Space Telescope. Here we report new JWST imaging, which clearly resolves MACS0647$-$JD as having two components that are either merging galaxies or stellar complexes within a single galaxy. Both are very small, with stellar masses $\sim10^8\,M_\odot$ and radii $r<100\,\rm pc$. The brighter larger component "A" is intrinsically very blue ($\beta\sim-2.6$), likely due to very recent star formation and no dust, and is spatially extended with an effective radius $\sim70\,\rm pc$. The smaller component "B" appears redder ($\beta\sim-2$), likely because it is older ($100-200\,\rm Myr$) with mild dust extinction ($A_V\sim0.1\,\rm mag$), and a smaller radius $\sim20\,\rm pc$. We identify galaxies with similar colors in a high-redshift simulation, finding their star formation histories to be out of phase. With an estimated stellar mass ratio of roughly 2:1 and physical projected separation $\sim400\,\rm pc$, we may be witnessing a galaxy merger 400 million years after the Big Bang. We also identify a candidate companion galaxy C $\sim3\,{\rm kpc}$ away, likely destined to merge with galaxies A and B. The combined light from galaxies A+B is magnified by factors of $\sim$8, 5, and 2 in three lensed images JD1, 2, and 3 with F356W fluxes $\sim322$, $203$, $86\,\rm nJy$ (AB mag 25.1, 25.6, 26.6). MACS0647$-$JD is significantly brighter than other galaxies recently discovered at similar redshifts with JWST. Without magnification, it would have AB mag 27.3 ($M_{UV}=-20.4$). With a high confidence level, we obtain a photometric redshift of $z=10.6\pm0.3$ based on photometry measured in 6 NIRCam filters spanning $1-5\rm\mu m$, out to $4300\,\r{A}$ rest-frame. JWST NIRSpec observations planned for January 2023 will deliver a spectroscopic redshift and a more detailed study of the physical properties of MACS0647$-$JD.

==> individual0.tex <==
% Filters
\begin{deluxetable*}{lllccccr}
\tablecaption{\label{tab:phy}Physical properties of two galaxies in MACS0647--JD, JDa and JDb estimated from \texttt{Bagpipes}}
\tablewidth{\columnwidth}
\tablehead{
\colhead{}&
\colhead{Age ($\rm Myr$)}&
\colhead{Stellar Mass (${\rm log}(M_{*}/M_{\odot})$)}&
\colhead{$A_{V}$}&
\colhead{Formation redshift}
}
\startdata
JD1a  &$102^{+135}_{-64}$& $8.00^{+0.25}_{-0.31}$ &  $0.02^{+0.03}_{-0.01}$ & $12.9$ \\
JD1b  & $204^{+147}_{-128}$ & $7.82^{+0.20}_{-0.28}$ &  $0.12^{+0.11}_{-0.07}$ & $16.6$
%Photometric Redshift &$10.39^{+0.04}_{-0.03}$ &$10.84^{+0.07}_{-0.07}$ 
\enddata
%\tablenotetext{a}{Observatory}
\end{deluxetable*}
%\tablecomments{From http://www.stsci.edu/{\HST}/campaigns/frontier-fields/{\HST}-Survey}


==> scraps.tex <==

as an overdensity of red galaxies 
It was spectroscopically confirmed to be a cluster at redshift $z = 0.566$ by \cite{WenHan15}.


Discovered by Wen et al. (2012) based on photometric redshifts in SDSS-III. 
Renamed in the PSZ2 catalog with coordinates given in decimal degrees (Alternate Name above).

 the Wen, Han, & Liu SDSS-III cluster catalog (WHL; Wen et al. 2012);
 
 



The Planck survey 
This cluster was ranked as the 31st most massive cluster in the Planck PSZ2 catalog with a Sunyaev-Zeldovich calculated mass of $M_{500} = 9\times 10^{14} M_{\odot}$.

WHL J013719.8-082841 (henceforth \WHL) was discovered in SDSS imaging as an overdensity of red galaxies by \cite{WHL12}, and its redshift was subsequently confirmed at $z = 0.566$ by \cite{WenHan15}. 
This cluster was ranked as the 31st most massive cluster in the Planck PSZ2 catalog with a Sunyaev-Zeldovich calculated mass of $M_{500} = 9\times 10^{14} M_{\odot}$.  



\cite{Salmon2020} discovered at 15\arcsec\ long arc at $z_{phot} = 6.2$ lensed by this cluster and dubbed it the Sunrise Arc, prompting follow-up observations with HST (GO 15842, P.I. Coe). 
These follow-up images included 5 additional orbits of ACS F814W imaging, and two orbits each of ACS F475W and WFC3/IR F110W imaging, and are presented in detail in \cite{Welch2022_earendel}. 
The Sunrise Arc is shown in Figure \ref{fig:sunrise-arc}, and each of its 7 small clump structures are labeled. 
Additionally, this arc contains an extremely magnified lensed star presented in \cite{Welch2022_earendel}.
\WHL received a total of 7 hours of observations in the IRAC 3.6 $\mu$m band, and 5 hours in the 4.5$\mu$m band. 


The massive galaxy cluster 
WHL J013719.8-082841
(RA = 01:37:25.0,
Dec = $-$08:27:25.0,
$z = 0.566$)

$M_{500} = 8.9 \pm 0.7$

WHL J24.3324-8.477

WHL0137-08

later confirmed at $z = 0.566$ (Wen et al. 2015)

Within the Sunrise Arc, \citep{Welch22_Earendel} 
also discovered Earendel,
an individual star (or star system) at $z \sim 6$ magnified by a factor of thousands.
%the Sunrise Arc and Earendel lensed by \WHL.
%, the most highly magnified galaxy 


has the potential

Ancillary science includes discoveries of new distant lensed galaxies.

lensing higher redshifts
key to discovering the first galaxies with JWST

----------------------------

* JWST

* HST

* lensing magnification

* Sunrise Arc + Earendel

* WHL0137

* RELICS

* JWST 2282

* lensing most distant galaxies

----------------------------


The most spectacularly lensed galaxies were discovered in large ground-based surveys such as SDSS
or in follow-up imaging of galaxy clusters.


offers two advantages to complement ``blank field'' surveys.
First, the magnification reveals smaller spatial scales unattainable without a larger telescope.

Where blank fields revealed star forming clumps several 100 pc across,
lensed fields 
The kpc scale clumps observed in \HST\ images
gave way to lensed star clusters seves

in so many shapes, colors, and sizes, each galaxy unique with its own story to tell.

Galaxies evolved over cosmic time from small irregular clumpy clusters and chains
to majestic spirals and ellipticals we see at present day in the local universe.
Hubble looked 97\% of the way back to the Big Bang, seeing $z = 11$ galaxies as they were
13.4 billion years ago when the universe was just 400 million years old.
% Spitzer


The Hubble Space Telescope (HST) revealed the beautiful diversity of galaxies
in so many shapes, colors, and sizes, each galaxy unique with its own story to tell.
Galaxies evolved over cosmic time from small irregular clumpy clusters and chains
to majestic spirals and ellipticals we see at present day in the local universe.
Hubble looked 97\% of the way back to the Big Bang, seeing $z = 11$ galaxies as they were
13.4 billion years ago when the universe was just 400 million years old.
% Spitzer



offers the promise of efficiently discovering more distant galaxies (e.g., Coe+)
and magnifying distant galaxies to reveal small structures on parsec scales
that we couldn't see otherwise (Johnson, Vanzella, Welch).


The James Webb Space Telescope (JWST) is our generation's next great leap in technology
offering even deeper, higher resolution images extending to longer infrared wavelengths.
Every JWST image surpasses the Hubble Deep Fields, 
transforming our understanding of distant galaxies, revealing exquisite details
including tiny parsec scale star forming regions and low surface brightness tidal features,
and the full census of stellar mass in each galaxy 
including older and dustier populations invisible to Hubble too red and redshifted.

